Automated Description Generation for Software Patches

Software patches are pivotal in refining and evolving codebases, addressing bugs, vulnerabilities, and optimizations. Patch descriptions provide detailed accounts of changes, aiding comprehension and collaboration among developers. However, manual description creation poses challenges in terms of time consumption and variations in quality and detail. In this paper, we propose PATCHEXPLAINER, an approach that addresses these challenges by framing patch description generation as a machine translation task. In PATCHEXPLAINER, we leverage explicit representations of critical elements, historical context, and syntactic conventions. Moreover, the translation model in PATCHEXPLAINER is designed with an awareness of description similarity. Particularly, the model is explicitly trained to recognize and incorporate similarities present in patch descriptions clustered into groups, improving its ability to generate accurate and consistent descriptions across similar patches. The dual objectives maximize similarity and accurately predict affiliating groups. Our experimental results on a large dataset of real-world software patches show that PATCHEXPLAINER consistently outperforms existing methods, with improvements up to 189% in BLEU, 5.7X in Exact Match rate, and 154% in Semantic Similarity, affirming its effectiveness in generating software patch descriptions.

==> 4.translation.tex <==
\section{Neural Machine Translation}

% Overview
Neural machine translation (NMT) is an approach to machine translation that uses a single
end-to-end neural network. The key benefit to the approach is that a single system can be trained directly on source and target text, no longer requiring the pipeline of specialized systems used in statistical machine translation. The neural network architecture is called a sequence-to-sequence model (seq2seq). Assuming we are given a source sentence x = {x1,..., xS} and a target sentence y = {y1,..., xT}. By using the chain rule, the conditional distribution can factorize from left-to-right (L2R) as:

\subsection{Transformers}

The Transformer is the same as the previous sequence-to-sequence model with an encoder-decoder pair. However, a Transformer model uses the attention mechanism within the encoder called the self-attention mechanism which helps us pass information effectively between the encoder-decoder pair in both directions.

The Transformer architecture was originally designed for translation. During training, the encoder receives input sentences in a certain language, while the decoder receives the same sentences in the desired target language. In the encoder, the attention layers can use all the words in a sentence. The decoder works sequentially and can only pay attention to the words in the sentence that it has already translated.


\subsection{Deep Pre-trained Encoder-Decoder}

\subsection{Large language models} 

Large language models use transformer models and are trained using massive datasets. This enables them to recognize, translate, predict, or generate text or other content. Large language models are composed of multiple neural network layers. Recurrent layers, feedforward layers, embedding layers, and attention layers work in tandem to process the input text and generate output content.

There are many large language models for code, such as CodeBERT, CodeT5, and Codex. In this paper, we finetune CodeLLama to generate commit messages.


